Relativistic Viscous Hydrodynamics for High Energy Heavy Ion Collisions

It has been over a decade since the first experimental data from gold nuclei collisions at the Relativistic Heavy Ion Collider suggested hydrodynamic behavior. While early ideal hydrodynamical models were surprisingly accurate in their predictions, they ignored that the large longitudinal velocity gradient meant that even small shear viscosity would produce large corrections to the transverse dynamics. In addition, much less was known about the equation of state predicted by lattice calculations of quantum chromodynamics, which predicts a soft region as the degrees of freedom change from quarks to hadrons but no first-order phase transition. Furthermore, the effects of late, dilute stage rescattering were handled within the hydrodynamic framework to temperatures where local kinetic equilibrium is difficult to justify. This dissertation presents a three-dimensional viscous hydrodynamics code with a realistic equation of state coupled consistently to a hadron resonance gas calculation. The code presented here is capable of making significant comparisons to experimental data as part of an effort to learn about the structure of experimental constraints on the microscopic interactions of dense, hot quark matter.

==> chapter8.tex <==
Hydrodynamics predicts the evolution of the density and collective velocity deterministically
for a system with a given initial condition.  By far the most common method
of initializing a hydrodynamics code is to provide 
the state of a system at a given time, though the equations do not demand that particular 
hypersurface.  In the case of relativistic heavy ion collisions, the procedure for producing 
these initial conditions is highly uncertain and a principle source of uncertainty 
in interpreting observables.

In the face of such uncertainty, one looks for relationships that properly predict scaling relationships
with simple models.  One particularly robust model is the Glauber model.  Originally, the 
goal of the model was to predict total cross-section factorization - that the cross-section for
collision between nuclei A and B was $\sigma_{AB} \sim \sqrt{\sigma_{AA} \sigma_{BB}}$.  
Subsequently, a Monte Carlo version of the model has been shown to predict the distribution
of event multiplicities based on simple geometric relationships and a few physically motivated 
parameters.

There are two classes of Glauber model.  In the first, one generates a smooth
profile based on density distributions that is fixed for a given impact parameter.
In the second, the finite number and fixed positions of the nucleons are taken into account
and a Monte Carlo procedure produces a fluctuating initial condition.
In either case, one begins with a distribution of nucleons within each
nucleus offset by in the transverse plane by the impact parameter.
The number density distribution is  generally a Woods-Saxon 
\begin{equation} \label{eq:WoodsSaxon}
\rho(r) = \rho_0 \left[1 + \exp^{(r-R)/\xi} \right]^{-1}
\end{equation}
where the nuclei are assumed to be spherically symmetric and described by a radius (R), 
diffusiveness ($\xi$), and normalization ($\rho_0$). 
In the Monte Carlo version, one then distributes nucleons by drawing from the
distribution $4 \pi r^2  \rho(r)$ for radial positions of the nucleons, and flat distributions
for the azimuthal angle and the cosine of the polar angle.  Draws are performed once 
for each nucleon in each nucleus involved in the collision.  
The nucleons are then assumed to be black discs in the transverse plane of radius given by 
the total proton-proton inelastic cross-section for the collision energy
of interest.  Collisions occur any time black discs overlap in the transverse plane with 
the longitudinal distribution ignored.  One generally counts both the total number of
pairwise collisions, the number of binary collisions ( $N_{BC}$),
and the number of nucleons participating in any collision , the number of wounded nucleons ($N_{WN}$).

The participant and collisional models differ where the areal nuclear density 
is larger than $\sigma_{\text{in}}^{-1}$.  To understand why,
consider a small region where one nucleus has four nucleons and its partner has only two, which
arises when $b \approx R$.  In this case the number of binary collisions would be eight, but the number
of wounded nucleons would be six. This actually underestimates the difference, since one
generally scales to half the number of wounded nucleons to recover the same behavior for
diffuse systems where there will be two wounded nucleons for each binary collision.

While the impact parameter is not known for any particular event, the smallest
impact parameters should correspond to the highest multiplicity events.  Geometrically 
it is clear that the change in probability of a particular impact parameter scales with the impact parameter,
$d\sigma  = 2 \pi b ~ db$, like circular shells for integration in polar coordinates.  
Integrating this equation and assuming that no collisions take place beyond a
maximum impact parameter, the total cross-section is related to the maximum
impact parameter by $b_{\text{max}} = \sqrt{\sigma_{T}/\pi}$.
Experimentally events are separated into centrality classes which are the percentile
of the total number of particles produced in a particular collision but reversed such 
that the 0-5\% centrality class corresponds to the 5\% of all events containing the
most particles.  As long as particle production falls monotonically with impact
parameter, the relationship between the centrality class and the impact parameter
should be 
\begin{equation}
 \frac{\% {\text{cent}}}{100} = \frac{\pi b^2}{ \sigma_T} = \left( \frac{b}{b_{\text{max}}} \right)^2.
 \end{equation}
This allows one to calculate the average number of participant nucleon pairs for
each centrality class, which one can compare to the total number of charged particles
produced. Experimentally, the number of charged particles observed at 
midrapidity scales very well with the number of participants up to center of mass
collision energies around $\sqrt{s} = 100$ GeV/A.  At $\sqrt{s} = 200$ GeV/A the deviation
from this scaling is $\sim5\%$ faster than linear, there are more observed charged particles
than predicted by the number of wounded nucleons, from 0-40\% centrality.
Some groups have suggested that this implies an increasing importance of hard processes
that might scale with the number of binary collisions and find that a mixture of 85\% participant
and 15\% collisional scaling reproduces data at this energy.

If total particle production scaling is predicted well the number of participants,
then the distribution of energy density in the transverse plane should be given
by the distribution of participants. This is done either smoothly or including 
fluctuations.  In order to include fluctuations, one places nucleons in each
nucleus by Monte Carlo according to each density distribution which are
offset by the impact parameter.  Nucleons are considered to collide if their
impact parameter is less than $b_{nn} \le \sqrt{\sigma_{\text{in}}/\pi}$.
To obtain the hot source, one assumes that each participant, or binary collision, contributes 
equally to the energy or entropy density in the form of a Gaussian in the transverse plane.
Depending on the extent of these Gaussians, this approach produces a lumpy initial profile.
This is not useful for the simulation at hand as fluctuations are not handled, 
but generally the fluctuations do not seem to enter into the averaged quantities that are of interest for this study.

An alternative approach would be to treat the density of nucleons as a smooth function.
By analogy to the black discs in the Monte Carlo method, one should consider the
overlap of the transverse areal density to be the joint probability of finding a nucleon
in each nucleus at some transverse position, often called the thickness function
\begin{equation} \label{eq:thickness}
T_A(x,y) = \displaystyle\int_{-\infty}^{+\infty} dz \rho_A (x,y,z).
\end{equation}
If one thought that each collision contributed 
equal to the density profile, then that joint probability would be proportional to the initial
density locally, so $\epsilon(x,y) = K \sigma_{\text{in}} T_A T_B$
where K is a constant to be determined by comparison to experimental data.  
To reproduce participant scaling, the density should be scaled to
\begin{eqnarray} \label{eq:partScaling}
\epsilon(x,y) &\propto& T_A \left[ 1 - \left(1 - \sigma T_B \right)^B \right] + T_B \left[ 1 - \left(1 - \sigma T_A \right)^A \right] \\
\epsilon(x,y) &\approx& \frac{K}{2} \left[ T_A \left( 1 - e^{-\sigma T_B} \right) + T_B \left( 1 - e^{-\sigma T_A} \right) \right]
\end{eqnarray}
where we assume that A and B are large.
The factor of two emphasizes that if both $T_A$ and $T_B$ are small, the normalization
should be the same as for binary collision scaling.

The second part of  Equation \ref{eq:partScaling} suggests
that the function behaves like symmetric penetration of the thickness functions -- that is,
$T_A$ is attenuated as it interacts passing through nucleus B and vice versa.
This is not exactly the case.
The addition of these two terms means that if $T_A >> T_B$, 
one of these terms still behaves like $\sigma_{\text{inel}}T_A T_B$ while the other 
is suppressed.  This means that doubling the larger thickness roughly doubles
the output density.  While this is what one expects from the wounded nucleon
picture, it seems likely that doubling the larger thickness would have a reduced 
effect.  

\begin{figure}
\centerline{\includegraphics[width=0.6 \textwidth]{ch6Figs/modelCompDensX.pdf}}
\caption{ 
(Color in electronic version)
Comparison along short axis between KLN, wounded nucleon, and simple saturation
models.
}
\label{fig:ICDensX}
\end{figure}

A model that would reduce the density in this scenario might scale to
\begin{equation} \label{eq:simpleSatIC}
\epsilon(x,y) = K \sigma \frac{2T_A T_B}{T_A+T_B} \left[ 1 - e^{-\sigma(T_A+T_B)/2} \right].
\end{equation}
We expect this to behave roughly as if one statistically removed participant nucleons
from consideration after each detected collision.
This model achieves the same scaling in the diffuse limit and generally
we expect the total density scaling to behave more like participant scaling
that collsional scaling. In fact, in regions where the thicknesses are similar
the model is the same as the wounded nucleon model.  But in regions where
the thicknesses are very different, such as where the tails of one nucleus
overlap with the center of the other nucleus in the transverse plane, this
will fall off much faster as seen in Figure \ref{fig:ICDensX}.

Other improvements to the Glauber model have been considered at impressive 
length by the PHOBOS collaboration including variation of nuclear density
profile parameters, the inelastic nucleon-nucleon cross-section, hardcore nucleon
repulsion within the original nucleus, and several experimental considerations
that would affect interpretation of the multiplicity results.  For reasonable variations
of the parameters, they find only $\pm 5\%$ influence on results for collisions mid-central
and central collisions for Au+Au collisions at $\sqrt{s} = 200$ GeV where
the largest deviations are for the experimental considerations.  Also of note
is that corrections for very peripheral collisions can be considerable larger, up to $\sim 20\%$.

Furthermore, they investigate differences between using smooth density profiles 
and using the average of many Monte-Carlo events to determine multiplicity scaling.  
They find that for mid-central collisions, smooth profiles predict $\sim 10\%$ fewer
particles produced by the 30-40\% centrality bin for Au+Au collisions at $\sqrt{s} = 130$ GeV.

